Data Structures for Approximate Discrete Fr\'echet Distance

The Fr\'{e}chet distance is a popular distance measure between curves $P$ and $Q$. Conditional lower bounds prohibit $(1 + \varepsilon)$-approximate Fr\'{e}chet distance computations in strongly subquadratic time, even when preprocessing $P$ using any polynomial amount of time and space. As a consequence, the Fr\'echet distance has been studied under realistic input assumptions, for example, assuming both curves are $c$-packed. In this paper, we study $c$-packed curves in Euclidean space $\mathbb R^d$ and in general geodesic metrics $\mathcal X$. In $\mathbb R^d$, we provide a nearly-linear time static algorithm for computing the $(1+\varepsilon)$-approximate continuous Fr\'echet distance between $c$-packed curves. Our algorithm has a linear dependence on the dimension $d$, as opposed to previous algorithms which have an exponential dependence on $d$. In general geodesic metric spaces $\mathcal X$, little was previously known. We provide the first data structure, and thereby the first algorithm, under this model. Given a $c$-packed input curve $P$ with $n$ vertices, we preprocess it in $O(n \log n)$ time, so that given a query containing a constant $\varepsilon$ and a curve $Q$ with $m$ vertices, we can return a $(1+\varepsilon)$-approximation of the discrete Fr\'echet distance between $P$ and $Q$ in time polylogarithmic in $n$ and linear in $m$, $1/\varepsilon$, and the realism parameter $c$. Finally, we show several extensions to our data structure; to support dynamic extend/truncate updates on $P$, to answer map matching queries, and to answer Hausdorff distance queries.

==> table.tex <==

\begin{table}[ht]
\vspace{1em}
    \centering
    \begin{tabular}{c|l|c|l| l|c}
   \textbf{Problem} & \textbf{Static solution} & \textbf{Source} & \textbf{Preprocessing} & \textbf{Query}  & Thm. \\
   \hline \hline
   \makecell{ deciding \frechet distance in $\X$ \\
   computing \frechet distance in $\X$} & - & - & -  & - & -\\
   \hline
   \makecell{$\X = \R^d$ -- $L_1, L_2, L_\infty$ \\
   real RAM with square roots} & 
   \makecell{ $O( d c n \log n + d \frac{c n}{ \sqrt{\eps}} \log \eps^{-1})$ \\
   $O( (d 2^d + c) n \log n + d \frac{cn}{\eps})$ 
   }
   & 
   $O( d n \log n )$ & \makecell{$O( d \frac{cm}{\eps})$ \\
   $O( d \frac{cm}{\eps} \log n )$} & \makecell{ Thm~\ref{thm:decidingfrechet} \\
   Thm.~\ref{thm:computingfrechet}}
   \makecell{\cite{bringmann2014improved} \\
   \cite{DriemelHW12}  } 
   \\
   -
    \end{tabular}
    \caption{
    All our results, for brevity, assume that $n > m$ (and thus $O(n + m) = O(n)$).
    \label{tab:results}
    }
\end{table}





\begin{proof}
The proof is by contradiction.
Suppose that the $j$'th row of $M^{P^{\mu} \times Q}_{\rho^*}$ contains strictly more than $\frac{c \cdot k}{\eps}$ $0$'s. 
Let $P' \subset P^\mu$ be the points which realise these zeros. I.e. the points $p_i \in P^\mu$ for which $d(p_i, q_j) \leq \rho^*$. 
Then $|P_i| > (1 + \eps) \cdot \frac{c \cdot k}{\eps} $
We consider the point $q_j \in Q$ and a ball $B$ in $\X$ with radius $(1 + \eps) \rho^*$. 
For each $p_i \in P'$, consider furthermore the segment $\ell_i$ of $P$ of length $\mu$ that immediately follows $p_i$.  
Per definition of $\mu$-compression, each of the segments $\ell_i$ do not (partially) coincide.
Moreover, each segment $\ell_i$ is contained within $B$ (since it has length at most $\mu \leq \eps \rho^*$). 
However, this lower bounds the length of $P \cap B$:
\[
\ell( P \cap B) \geq \sum_{p \in P'} \mu > (1 + \eps) \cdot \frac{c \cdot k}{\eps} \cdot \mu = (1 + \eps) \cdot c \cdot \rho^* = c \cdot |B|.
\]
This contradicts the assumption that $P$ was $c$-packed. 
\end{proof}
